Safety-Constrained Model Predictive Control for an Omnidirectional Walking Assistive Robot Using Control Barrier Function

Providing safe and effective mobility assistance plays a crucial role in restoring independence and enhancing the quality of life for individuals with motor impairments. In this context, robotic walking assistive devices have recently emerged as promising solutions to provide physically compliant interaction while ensuring user safety and support. This paper presents a novel control framework for an omnidirectional Walking Assistive Robot (I-WANDER) that integrates a Control Barrier Function (CBF) formulation into a Model Predictive Control (MPC) scheme to explicitly enforce collision-avoidance safety constraints while optimizing for energy efficiency and smooth human-robot collaboration. The method was experimentally evaluated with 12 healthy participants performing two different walking tasks using both the proposed CBF-based MPC controller (CB-MPC) and a variable admittance controller (AC). The first task involved structured navigation through a U-shaped corridor, whereas the second consisted of a single-obstacle avoidance task performed blindfolded to ensure the obstacle was unexpected. Comparative results show that the CB-MPC architecture significantly reduces energy consumption and mechanical work (p < 0.01) without compromising motion smoothness, while also decreasing the number of obstacle collisions. Overall, the findings highlight the potential of the proposed control architecture to enhance both safety and efficiency in robotic walking assistance.

==> Method/mpc_formulation.tex <==
\section{Linear MPC with Rectangular CBF Constraints}
\label{sec:lmpc_cbf}

\subsection{Discrete-time local-frame model}
We consider a prediction horizon $N$ and sampling time $\Delta t$. The robot state and control input are
\begin{equation}
x_k \triangleq 
\begin{bmatrix}
p_{x,k} & p_{y,k} & \theta_k
\end{bmatrix}^\top \in \mathbb{R}^3,
\qquad
u_k \triangleq
\begin{bmatrix}
v_{x,k} & v_{y,k} & \omega_k
\end{bmatrix}^\top \in \mathbb{R}^3,
\label{eq:state_input_def}
\end{equation}
where $u_k$ is expressed in the robot \emph{local} frame. Under the local-frame kinematic model used in our implementation, the dynamics are linear:
\begin{equation}
x_{k+1} = x_k + \Delta t\,u_k,\qquad k=0,\dots,N-1,
\label{eq:local_linear_dynamics}
\end{equation}
with initial condition $x_0=\hat{x}_0$ provided by the reference/estimator.

\subsection{Quadratic objective}
Given reference trajectories $\{x_k^{\mathrm{ref}}\}_{k=0}^N$ and (optionally) $\{u_k^{\mathrm{ref}}\}_{k=0}^{N-1}$, we use a standard quadratic tracking cost
\begin{equation}
\ell_k(x_{k+1},u_k) \triangleq 
\|x_{k+1}-x_{k+1}^{\mathrm{ref}}\|_{Q}^2 + \|u_k-u_k^{\mathrm{ref}}\|_{R}^2,
\label{eq:stage_cost}
\end{equation}
where $\|e\|_{Q}^2 \triangleq e^\top Q e$, $Q\succeq 0$, $R\succ 0$.
Optionally, an additional prediction-tracking term $\|x_{k}-x_{k}^{\mathrm{pred}}\|_{Q_2}^2$ can be included if a learned predictor is available.

To discourage aggressive transients, we add a quadratic jerk regularizer based on second differences of the input:
\begin{equation}
\Delta u_k \triangleq u_k-u_{k-1},\qquad 
\Delta^2 u_k \triangleq \Delta u_k-\Delta u_{k-1}.
\label{eq:jerk_defs}
\end{equation}
The corresponding penalty is $\|\Delta^2 u_k\|_{J}^2$ with $J\succeq 0$. For $k=0,1$, the differences are initialized using the previously applied control $u_{-1}$ and/or a stored estimate of past acceleration, as done in the implementation.

\subsection{Rectangular obstacle model and active-face selection}
We model each obstacle $j\in\{1,\dots,N_o\}$ as an \emph{unsafe rectangular region} in the robot local frame.
Let $(u_j,v_j)\in\mathbb{R}^2$ denote the obstacle position expressed in the robot local frame and \emph{frozen at the current time} (i.e., held constant across the horizon during one MPC solve). Let $a>0$ and $b>0$ denote the rectangle half-length and half-width (robot footprint possibly inflated).

To avoid mixed-integer optimization, we activate only one rectangle face per obstacle by selecting, outside the optimizer, the parameters
\begin{equation}
\alpha_{k,j}\in\{0,1\},\qquad s^u_{k,j}\in\{-1,1\},\qquad s^v_{k,j}\in\{-1,1\},
\label{eq:face_params}
\end{equation}
where $\alpha_{k,j}=1$ selects a vertical face ($u$-face) and $\alpha_{k,j}=0$ selects a horizontal face ($v$-face), while $s^u_{k,j}$ and $s^v_{k,j}$ select the sign (left/right or bottom/top). In practice, $\{\alpha_{k,j},s^u_{k,j},s^v_{k,j}\}$ are computed via a proximity rule with hysteresis and passed to the MPC as parameters.

\subsection{Local rectangular ZCBF constraint (affine in the decision variables)}
We adopt a zeroing CBF (ZCBF) condition. For obstacle $j$ at step $k$, define a one-face barrier function
\begin{equation}
h_{k,j} \triangleq 
\alpha_{k,j}\big(s^u_{k,j}u_j-a\big)+
(1-\alpha_{k,j})\big(s^v_{k,j}v_j-b\big),
\label{eq:rect_barrier}
\end{equation}
which is constant during the QP solve because $(u_j,v_j)$ and the face parameters are frozen.

Assuming obstacles are static in the world, their relative motion in the robot local frame induced by the robot command $u_k$ is
\begin{equation}
\dot u = -v_{x,k} + \omega_k\,v_j,\qquad 
\dot v = -v_{y,k} - \omega_k\,u_j.
\label{eq:relative_kinematics}
\end{equation}
The barrier derivative for the selected face is
\begin{equation}
\dot h_{k,j} =
\alpha_{k,j}s^u_{k,j}\dot u + (1-\alpha_{k,j})s^v_{k,j}\dot v.
\label{eq:hdot_def}
\end{equation}
Substituting \eqref{eq:relative_kinematics} into \eqref{eq:hdot_def} yields an affine function of $u_k$.
To keep expressions compact in two columns, we define coefficients component-wise:
\begin{equation}
\begin{aligned}
a^{(x)}_{k,j} &\triangleq -\alpha_{k,j}s^u_{k,j},\\
a^{(y)}_{k,j} &\triangleq -(1-\alpha_{k,j})s^v_{k,j},\\
a^{(\omega)}_{k,j} &\triangleq 
\alpha_{k,j}s^u_{k,j}v_j-(1-\alpha_{k,j})s^v_{k,j}u_j,
\end{aligned}
\label{eq:cbf_coeffs}
\end{equation}
so that
\begin{equation}
\dot h_{k,j} =
a^{(x)}_{k,j}v_{x,k} + a^{(y)}_{k,j}v_{y,k} + a^{(\omega)}_{k,j}\omega_k
= \mathbf{a}_{k,j}^\top u_k,
\label{eq:hdot_affine}
\end{equation}
with $\mathbf{a}_{k,j}\triangleq[a^{(x)}_{k,j}\;\;a^{(y)}_{k,j}\;\;a^{(\omega)}_{k,j}]^\top$.

The ZCBF inequality is enforced as
\begin{equation}
\dot h_{k,j} + \gamma\,h_{k,j} \ge 0,\qquad \gamma>0.
\label{eq:zcbf_rect}
\end{equation}
Optionally, to guarantee feasibility in cluttered environments, we soften \eqref{eq:zcbf_rect} with a nonnegative slack $\sigma_k\ge 0$:
\begin{equation}
\dot h_{k,j} + \gamma\,h_{k,j} + \sigma_k \ge 0,
\qquad \sigma_k\ge 0.
\label{eq:zcbf_rect_slack}
\end{equation}
Since $h_{k,j}$ and $\mathbf{a}_{k,j}$ are parameters during the solve, \eqref{eq:zcbf_rect}--\eqref{eq:zcbf_rect_slack} are linear inequalities in the decision variables.

\subsection{QP formulation of the CBF-MPC problem}
Let $\mathcal{K}\triangleq\{0,\dots,M-1\}$ denote the set of steps where CBF constraints are enforced (typically $M=N$), and $\mathcal{O}\triangleq\{1,\dots,N_o\}$ denote the obstacle indices. The optimization variables are the state trajectory $\{x_k\}_{k=0}^N$, control trajectory $\{u_k\}_{k=0}^{N-1}$, and (if enabled) slack variables $\{\sigma_k\}_{k=0}^{M-1}$.

The resulting convex QP is
\begin{subequations}\label{eq:cbf_mpc_qp}
\begin{IEEEeqnarray}{rCl}
\min_{\{x_k,u_k,\sigma_k\}}
&& \sum_{k=0}^{N-1}\ell_k(x_{k+1},u_k)
+ \sum_{k=0}^{N-1}\|\Delta^2 u_k\|_{J}^2
+ w_\sigma\sum_{k=0}^{M-1}\sigma_k^2
\label{eq:cbf_mpc_cost}\\
\text{s.t.}
&& x_{k+1}=x_k+\Delta t\,u_k,\quad x_0=\hat{x}_0,\quad k=0,\dots,N-1
\label{eq:cbf_mpc_dyn}\\
&& u_{\min}\le u_k \le u_{\max},\quad k=0,\dots,N-1
\label{eq:cbf_mpc_ubounds}\\
&& \mathbf{a}_{k,j}^\top u_k + \gamma\,h_{k,j} + \sigma_k \ge 0,
\quad k\in\mathcal{K},\; j\in\mathcal{O}
\label{eq:cbf_mpc_cbf}\\
&& \sigma_k \ge 0,\quad k\in\mathcal{K}.
\label{eq:cbf_mpc_slack}
\end{IEEEeqnarray}
\end{subequations}
Additional linear constraints, such as bounds on input increments
$\Delta u_{\min}\le u_k-u_{k-1}\le \Delta u_{\max}$ and/or state bounds
$x_{\min}\le x_k\le x_{\max}$, can be included without altering convexity.

\paragraph{Convexity and solver choice.}
The objective \eqref{eq:cbf_mpc_cost} is quadratic with positive semidefinite Hessian, while
\eqref{eq:cbf_mpc_dyn}--\eqref{eq:cbf_mpc_slack} are linear equalities/inequalities because obstacle positions and active faces are treated as parameters.
Therefore, \eqref{eq:cbf_mpc_qp} is a convex QP that can be solved efficiently with sparse QP solvers (e.g., OSQP) for real-time control.

==> Method/mpc_formulation_compact.tex <==
% ============================================================
% RAL-ready compact QP form (stacked variables)
% Linear MPC + rectangular ZCBF constraints (local frame, frozen obstacles)
% ============================================================

\subsection{Compact QP Formulation (Stacked Variables)}
\label{sec:compact_qp}

We cast the proposed CBF-MPC problem as a standard convex quadratic program (QP)
\begin{equation}
\min_{z}\ \frac{1}{2} z^\top H z + q^\top z
\quad \text{s.t.}\quad
A z = b,\ \ G z \le g,
\label{eq:qp_standard_form}
\end{equation}
where the decision vector $z$ stacks the full state trajectory, input trajectory, and slack variables.

\subsubsection{Stacked decision variables}
Let $N$ denote the MPC horizon, $M\le N$ the number of steps at which CBF constraints are enforced, and $n=m=3$.
We define the stacked vectors
\begin{equation}
X \triangleq 
\begin{bmatrix}
x_0^\top & x_1^\top & \cdots & x_N^\top
\end{bmatrix}^\top \in \mathbb{R}^{(N+1)n},
\qquad
U \triangleq
\begin{bmatrix}
u_0^\top & u_1^\top & \cdots & u_{N-1}^\top
\end{bmatrix}^\top \in \mathbb{R}^{Nm},
\label{eq:stack_XU}
\end{equation}
and the nonnegative slack vector
\begin{equation}
\Sigma \triangleq
\begin{bmatrix}
\sigma_0 & \sigma_1 & \cdots & \sigma_{M-1}
\end{bmatrix}^\top \in \mathbb{R}^{M}.
\label{eq:stack_Sigma}
\end{equation}
The overall decision vector is
\begin{equation}
z \triangleq
\begin{bmatrix}
X^\top & U^\top & \Sigma^\top
\end{bmatrix}^\top.
\label{eq:z_def}
\end{equation}

\subsubsection{Quadratic cost in matrix form}
The stage cost is
\(
\ell_k = (x_{k+1}-x_{k+1}^{\mathrm{ref}})^\top Q (x_{k+1}-x_{k+1}^{\mathrm{ref}})
+ (u_k-u_k^{\mathrm{ref}})^\top R (u_k-u_k^{\mathrm{ref}})
\)
and we additionally penalize slack with $w_\sigma>0$.
Define the block-diagonal matrices
\begin{equation}
\bar{Q} \triangleq \mathrm{blkdiag}(\underbrace{0,\ Q,\ \dots,\ Q}_{N\ \text{times}}) \in \mathbb{R}^{(N+1)n \times (N+1)n},
\qquad
\bar{R} \triangleq \mathrm{blkdiag}(\underbrace{R,\ \dots,\ R}_{N\ \text{times}}) \in \mathbb{R}^{Nm \times Nm},
\label{eq:Qbar_Rbar}
\end{equation}
where the first block of $\bar Q$ is set to zero since the cost starts at $x_1$.
Let
\begin{equation}
X^{\mathrm{ref}} \triangleq
\begin{bmatrix}
(x_0^{\mathrm{ref}})^\top & \cdots & (x_N^{\mathrm{ref}})^\top
\end{bmatrix}^\top,
\qquad
U^{\mathrm{ref}} \triangleq
\begin{bmatrix}
(u_0^{\mathrm{ref}})^\top & \cdots & (u_{N-1}^{\mathrm{ref}})^\top
\end{bmatrix}^\top,
\label{eq:ref_stacks}
\end{equation}
and $\bar{W}_\sigma \triangleq w_\sigma I_M$.
Then the objective can be written as
\begin{equation}
J(z) =
\frac{1}{2} X^\top (2\bar Q) X - (2\bar Q X^{\mathrm{ref}})^\top X
+
\frac{1}{2} U^\top (2\bar R) U - (2\bar R U^{\mathrm{ref}})^\top U
+
\frac{1}{2}\Sigma^\top (2\bar W_\sigma)\Sigma
+ \text{const}.
\label{eq:cost_expand}
\end{equation}
Therefore, \eqref{eq:qp_standard_form} holds with
\begin{equation}
H = \mathrm{blkdiag}(2\bar Q,\ 2\bar R,\ 2\bar W_\sigma),
\qquad
q =
\begin{bmatrix}
-2\bar Q X^{\mathrm{ref}}\\[2pt]
-2\bar R U^{\mathrm{ref}}\\[2pt]
\mathbf{0}
\end{bmatrix}.
\label{eq:H_q_def}
\end{equation}
(Any constant term can be dropped.)

\subsubsection{Dynamics equalities as $Az=b$}
The local-frame linear model is
\(
x_{k+1} = x_k + \Delta t\,u_k
\).
Let $A_d \triangleq I_n$ and $B_d \triangleq \Delta t\,I_n$.
For each $k=0,\dots,N-1$ we impose
\(
x_{k+1}-A_d x_k - B_d u_k = 0
\)
and the initial condition
\(
x_0=\hat x_0
\).
Stacking these equalities yields
\begin{equation}
A z = b,
\label{eq:Azb}
\end{equation}
where $A$ is the sparse banded matrix encoding the $N$ dynamics constraints and the initial condition, acting only on the $(X,U)$ blocks of $z$ (the $\Sigma$ block does not appear in $Az=b$).

\subsubsection{Rectangular ZCBF inequalities as $Gz\le g$}
We enforce rectangular ZCBF constraints for $N_o$ obstacles over steps $k\in\mathcal{T}\triangleq\{0,\dots,M-1\}$.
Obstacle $j$ is represented in the robot local frame by its frozen coordinates $(u_j,v_j)$.
An external routine selects active-face parameters
$\alpha_{k,j}\in\{0,1\}$ and $s^u_{k,j},s^v_{k,j}\in\{-1,1\}$.

The one-face barrier value is
\begin{equation}
h_{k,j} =
\alpha_{k,j}(s^u_{k,j}u_j-a) + (1-\alpha_{k,j})(s^v_{k,j}v_j-b),
\label{eq:h_kj_param}
\end{equation}
which is constant during the QP solve.
Using the relative kinematics, the barrier derivative is affine in $u_k$:
\begin{equation}
\dot h_{k,j} = \mathbf{a}_{k,j}^\top u_k,
\label{eq:hdot_affine_compact_form}
\end{equation}
where $\mathbf{a}_{k,j}\in\mathbb{R}^3$ is a known coefficient vector computed from $(u_j,v_j,\alpha_{k,j},s^u_{k,j},s^v_{k,j})$.

The softened ZCBF inequality is
\begin{equation}
\mathbf{a}_{k,j}^\top u_k + \gamma h_{k,j} + \sigma_k \ge 0,\qquad \sigma_k\ge 0.
\label{eq:zcbf_soft}
\end{equation}
To fit the standard form $Gz\le g$, we rewrite \eqref{eq:zcbf_soft} as
\begin{equation}
-\mathbf{a}_{k,j}^\top u_k - \sigma_k \le \gamma h_{k,j},
\qquad \forall k\in\mathcal{T},\ \forall j\in\{1,\dots,N_o\}.
\label{eq:zcbf_soft_leq}
\end{equation}

Each inequality \eqref{eq:zcbf_soft_leq} becomes one row of $Gz\le g$.
In particular, the row places $-\mathbf{a}_{k,j}^\top$ in the columns of $U$ corresponding to $u_k$,
places $-1$ in the column of $\Sigma$ corresponding to $\sigma_k$, and zeros elsewhere.
The right-hand side entry is $g_{(k,j)}=\gamma h_{k,j}$.

\subsubsection{Additional linear constraints (optional)}
Input bounds $u_{\min}\le u_k\le u_{\max}$, input increment bounds
$\Delta u_{\min}\le u_k-u_{k-1}\le \Delta u_{\max}$, and state bounds
$x_{\min}\le x_k\le x_{\max}$ can be added by appending rows to $Gz\le g$.
The slack nonnegativity constraints are
\begin{equation}
-\Sigma \le 0,
\label{eq:slack_nonneg}
\end{equation}
and are also included in $Gz\le g$.

\paragraph{Convexity.}
Since $H\succeq 0$ (block diagonal with $Q\succeq 0$, $R\succ 0$, and $w_\sigma I\succeq 0$), and all constraints are linear,
\eqref{eq:qp_standard_form} is a convex QP and can be solved efficiently by sparse QP solvers.

==> Related_works/Introduction.tex <==

Gait dysfunction represents one of the most common causes of disability in Europe, with approximately five million citizens depending on a wheelchair. The progressive ageing of the global population further exacerbates this condition, as chronic diseases associated with ageing lead to an increasing prevalence of gait impairments and mobility-related disabilities. These limitations significantly reduce individuals’ ability to perform activities of daily living (ADLs) and to actively participate in social and professional life \cite{Tadeusz_review}.

To restore, support, and preserve mobility among elderly individuals, several mechanical assistive devices for gait support have been developed, including walkers and canes. However, traditional assistive tools present several limitations, such as the requirement of sufficient user-generated force to maneuver the device, limited adaptability to human motion, and the lack of robust support for user stability.

In recent years, robotic-assisted devices have emerged as a promising alternative to conventional ambulation tools. Most systems are designed as robotic canes or smart walkers composed of a mobile base and a handle interface \cite{xing2021admittance, ding2022intelligent, itadera2019predictive, itadera2022admittance}. Despite their technological advancements, these platforms typically rely on user-applied forces on the handlebars to generate motion commands. Moreover, they do not physically support the user’s trunk and therefore cannot prevent vertical falls; in the event of slipping, their ability to arrest the fall may be limited.

To address these shortcomings, reduced-dimension robotic platforms capable of physically supporting the user at the trunk level have recently been proposed to prevent falls. The mobile robotic balance assistant (MRBA) introduced in \cite{li2023mobile} implements a user-following strategy based on tracking the user’s Center of Mass (CoM) relative to the robot. When the robot--CoM distance exceeds a predefined threshold, the robot moves toward the user. 

Similarly, \cite{mun2014design, mun2015development, aguirre2019high, aguirre2021omnidirectional} proposed an omnidirectional assistive platform equipped with an admittance controller, which ensures smoother human–robot interaction compared to purely user-following approaches. As in the Andago system, these platforms rely on force/torque (FT) sensors coupled to the patient to measure interaction forces, which are then converted into desired velocities through an admittance model.

Nevertheless, assistive controllers—especially those deployed on platforms intended for users with motor impairments, who may exhibit involuntary or uncoordinated movements—must also guarantee collision avoidance and risk reduction. Individuals with gait disabilities often present not only sensorimotor deficits, reduced muscle strength, impaired coordination, and limited effort capacity, but also varying degrees of cognitive impairment, pain, and movement-avoidance strategies \cite{Tadeusz_review}. Therefore, the control strategy must explicitly account for constrained operational scenarios and ensure safe interaction with surrounding obstacles and humans. Notably, none of the aforementioned works explicitly addresses the problem of obstacle avoidance in trunk-support walking assistive devices.

In this work, we integrate obstacle avoidance capabilities through Control Barrier Functions (CBFs) embedded within a Model Predictive Control (MPC) framework. The proposed approach ensures safe ambulation with the A-ROBOT walking assistive device while simultaneously promoting effortless user locomotion. In doing so, this study addresses the current gap in the literature regarding formal obstacle avoidance strategies for trunk-support robotic walking assistance platforms.

==> Related_works/Related_works.tex <==

\subsection{Constraints based approach} 
Several NMPC approaches
use constraints on the maneuverable space according to
the current and predicted position of humans \cite{nair2022stochastic}.
However, constraining NMPC can make it hard to find a
feasible solution to the motion planning problem in cluttered
dynamic environments. 
Complex situations potentially cause constraint-based NMPC
approaches to freeze the robot (i.e., stopping the robot) due to
a large number of collision avoidance constraints being active
at the same time (e.g., due to optimizers returning infeasible
solutions). MMCA-NMPC (Rudenko work) utilizes a new collision avoidance
cost formulation based on stochastic multi-modal human
motion predictions \cite{Rudenko2023}
\subsection{Cost based approach} 
A cost term in the objective function does not impose any hard constrains which can cause the infeasibility of the problem but cannot provide formal safety guarantees. 
Constraint-based approaches guarantee that the optimal solution does not violate the defined constraints. However, a
high number of constraints also increases the computational
complexity of the nonlinear program. Most importantly,
constraints also introduce the possibility that the optimizer
is not able to find a solution to the program, thus resulting
in an infeasible iteration.
\subsection{Control Barrier Function}
Recently, CBF was introduced in [16], where the control input was
the solution to a quadratic programming problem. The main
idea of the quadratic programming program is to impose
a minimal invasive change of the stabilizing controller to
be also safe [17], [21]. However, those contributions lack
the prediction capabilities in the formulation of the MPC formulation. Recent efforts considered unifying CBF with traditional MPC formulation. \cite{ali2024linear}.
To the best of the authors’ knowledge, in the existing literature on mobile platforms, numerous works delve into obstacle avoidance; however, these primarily address autonomous [38] or semi-autonomous operations in a teleoperation setup [39], leaving aside physical human–robot interaction tasks such as co-transportation, which is the focus of the present work.

This work integrates a CBF within the MPC formulation in human-robot physical collaboration framework. In particular the proposed method ensure safe ambulation with a walking assistive device while promoting effortless user locomotion, colmando il gap sull'assenza di metodi per obstacle avoidance in dispositivi di assistenza alla camminata presentati nella letteratura.

% \subsection{Contribute of the paper}
In this study a introduces WANDER, a novel Walking Assistive
omNi-Directional Exo-Robot1 with a personalizable controller.
It consists of a mobile omnidirectional platform that ensures
free movements on the ground, a robust BWS aluminum
structure on top of it, and a comfortable and minimally
restrictive coupling interface provided with an FT sensor
to detect the users’ intentions. To evaluate A-ROBOT’s effectiveness in reducing energy consumption while maintaining a smooth human-robot interaction user performance and comfort against the existing approaches, we conducted experiments with twelve subject

